An Efficient and Robust Committee Structure for Sharding Blockchain

Nowadays, sharding is deemed as a promising way to save traditional blockchain protocols from their low scalability. However, such technique also brings several potential risks and huge communication overheads. An improper design may give rise to the inconsistent state among different committees. Further, the communication overheads arising from cross-shard transactions unfortunately reduce the system's performance. In this paper, we first summarize five essential issues that all sharding blockchain designers face. For each issue, we discuss its key challenge and propose our suggested solutions. In order to break the performance bottlenecks, we propose a reputation mechanism for selecting leaders. The term of reputation in our design reflects each node's honest computation resources. In addition, we introduce a referee committee and partial sets in each committee, and design a recovery procedure in case the leader is malicious. Under the design, we prove that malicious leaders will not hurt the system and will be evicted. Furthermore, we conduct a series of simulations to evaluate our design. The results show that selecting leaders by the reputation can dramatically improve the system performance.

==> Performance.tex <==
\section{Performance Analysis}\label{sec:performance}

We claim that our protocol is efficient in intra-shard and cross-shard transactions processing. 

Recall that we use $n$ to denote the number of nodes in the network, $m$ to denote the number of committees and $c$ to denote the expected amount of participants in a committee.

\subsection{Complexity of Committee Configuration}

In this phase, all members in any committee except $C_R$ will recognize each other, which imposes a communication, computation and storage complexity of $O(c)$ for all common members. For leaders and partial set members, the communication complexity is multiplied by $c$ as each of them has to deliver $i$ pieces of information to the $i^{th}$ applying participant.

\subsection{Complexity of Commitment Exchanging}

For any leader, he/she is obliged to produce the commitment of his/her committee and note down commitments from all other committees. Thus, the computation complexity is $O(c)$ while the storage complexity is $O(m)$. However, members in $C_R$ has to suffer from the huge transportation overhead of $O(m^2)$ as they have to propagate all commitments to all committees as intermediaries.

\subsection{Complexity of Reaching Intra-committee Consensus}

To reach a consensus on a set of transactions with constant size, one in a committee has to broadcast the set with his/her signature to all members in a committee, which causes a communication complexity of $O(c)$. For key members, they must store the information with at least half of the members' certification to acknowledge the set, hence, a storage complexity of $O(c)$ is induced. At the same time, common members only need to keep their own opinion in reserve. 

\subsection{Complexity of Block Generation and Propagation}

To propose a block with size $O(n)$ and broadcast it to all committees, an $O(mn)$ communicating burden and an $O(n)$ storage overhead are inevitable for any participant in $C_R$. However, we point out that the expense also exists in almost all previous protocols. At the same time, for any other attendee, the storage complexity is just $O(c)$, as he/she only needs to maintain the participants, transactions, and UTXOs within the committee he/she belongs to.

We summarize the theoretical analysis of the performance of CycLedger in Table~\ref{Complexity}.

\begin{table*}[!t]
    \renewcommand{\arraystretch}{1.35}
    \caption{Communication, Computation \& Storage Complexity of CycLedger}
    \label{Complexity}
    \centering
    \begin{threeparttable}
        \begin{tabular}{|c|c|c|c|c|}
           \hline
             Communication \& Computation / Storage Complexity & Common Members & Leaders \& Partial Set Members & $C_R$ Members \\
          \hline
             Committee Configuration & $O(c) / O(c)$ & $O(c^2) / O(c^2)$ & - \\
            \hline
            Semi-Commitment Exchanging & - & $O(c) / O(m)$ & $O(m^2) / O(m)$ \\
            \hline
            Intra-committee Consensus & $O(c) / O(1)$ & $O(c) / O(c)$ & $O(n) / O(n)$  \\
            \hline
            Inter-committee Consensus & $O(m) / O(1)$ & $O(n) / O(1)$ & $O(n) / O(n)$  \\
            \hline
            Reputation Updating & $O(c) / O(1)$ & $O(c) / O(c)$ & $O(n) / O(n)$  \\
            \hline
            Key Member Selection & - & - & $O(n) / O(n)$  \\
            \hline
            Block Generation \& Propagation & $O(m) / O(c)$ & $O(n) / O(c)$ & $O(mn) / O(n)$  \\
            \hline
        \end{tabular}
        \begin{tablenotes}
           \footnotesize
           \item[1] $n$: total amount of nodes in the network\ $m$: amount of committees\ $c$: amount of nodes in a committee, we mention again that $n = mc$.
        \end{tablenotes}
    \end{threeparttable}
\end{table*}
